AdapMoE: Adaptive Sensitivity-based Expert Gating and Management for Efficient MoE Inference

Mixture-of-Experts (MoE) models are designed to enhance the efficiency of large language models (LLMs) without proportionally increasing the computational demands. However, their deployment on edge devices still faces significant challenges due to high on-demand loading overheads from managing sparsely activated experts. This paper introduces AdapMoE, an algorithm-system co-design framework for efficient MoE inference. AdapMoE features adaptive expert gating and management to reduce the on-demand loading overheads. We observe the heterogeneity of experts loading across layers and tokens, based on which we propose a sensitivity-based strategy to adjust the number of activated experts dynamically. Meanwhile, we also integrate advanced prefetching and cache management techniques to further reduce the loading latency. Through comprehensive evaluations on various platforms, we demonstrate AdapMoE consistently outperforms existing techniques, reducing the average number of activated experts by 25% and achieving a 1.35x speedup without accuracy degradation. Code is available at: https://github.com/PKU-SEC-Lab/AdapMoE.

==> docs/cache.tex <==
\section{DP Formulation}


\begin{table}
    \centering
    \caption{Notations used in the DP Fomulation }
    \begin{tabular}{|c|c|} \hline 
         Name& Meaning\\ \hline 
         T& Total expert capcity\\ \hline 
         $\alpha_i$& Expert cache hit probability of layer i\\ \hline 
         $\beta_i$& Expert prediction accuracy of layer i\\ \hline 
         $\gamma_i$& Probablity of only executing one expert of layer i\\ \hline
    \end{tabular}
    \label{tab:my_label}
\end{table}

==> docs/outline.tex <==
\section{outline}

\begin{itemize}
    \item Mixture-of-Experts (MoE) models are designed to relieve the high compute requirements of Large Language Models (LLMs). The feedforward block in MoE selects from a variety of distinct parameter groups using a gating function, which enables MoE to scale its model size without proportionally scaling up its computational requirements. For instance, in the Mixtral-8x7b model, each token can access 47 billion parameters, yet only 13 billion active parameters are utilized during each inference iteration.
    \item Unfortunately, the substantial memory requirements of MoE makes it difficult to be deployed, especially on edge devices with limited memory. One typical solution is offloading. The weights of the experts are stored on CPU memory, SSDs, or Flash storage, and will only be loaded into the GPU when needed for computations. However, the approach of dynamically migrating activated experts on-demand leads to the serialization of the expert selection phase with the expert execution phase, thereby introducing significant performance overhead.
    \item Faced with these challenges, existing works have explored several expert caching and prefetching algorithm. 
        \begin{itemize}
            \item Mixtral-offloading\cite{} observes token-wise expert selection affinity and adopts LRU algorithm to manage the expert cache. Each layer has the same expert cache size for convenience.
            \item MoE-Infinity\cite{} observes layer-wise expert selection affinity. It collects typical expert activation patterns into LUTs and then executes prefetching based on the LUT prediction.
            \item Pre-gated Moe\cite{} modifies the structure of MoE, in which the experts are selected based on the previous layers' activation. It enables the activated experts to be prefetched one layer ahead.
        \end{itemize}
    \item Motivation
        \begin{itemize}
            \item \textbf{Target: Minimize on-demand expert loading overhead/frequency}
            \item Mixtral-offloading and MOE-INFINITY both face the challenge of low prediction accuracy, for their caching and prefetching algorithm are merely based on expert activation statistics.
            \item Pre-gated MoE ensures accurate prefetching of the correct experts. However, this modification necessitates adjustments to the model's architecture and subsequent fine-tuning, which complicates the convenient deployment of open-source large MoE models. Severely, it only predicts and prefetches next layers' experts. \textit{The prefetch may not be fully overlapped without global scheduling.}
        \end{itemize}
    \item Observation
        \begin{itemize}
            \item \textbf{Dynamic expert Demands.} Exisiting MoE models select same number of experts for each tokens in each layer, regardless the weight distribution. We find it sub-optimal. \textit{Intuitively, some exactly classified tokens only needs to select one expert.} Thus, the on-demand loading of experts can be reduced directly.
            \item \textbf{Similar intermediate activation}. The activations between successive layers exhibit a very high degree of similarity. This characteristic is due to the nature of the residual connections, which aim to propagate the original input features across layers with minimal alteration, thus maintaining a consistency in the feature space as the depth increases. 
            \item \textbf{Unbalanced expert cache demands.} We find that the earlier layers prefer to select more experts, and are harder to predict the selection of experts. While the later layers prefer to select fewer experts, and are easier to predcit the selection of experts. Thus, their demands for expert cache are different.
        \end{itemize}
    \item Main Contribution
        \begin{itemize}
            \item \textbf{Dynamic expert selection.}
            \item \textbf{Reuse-based pre-gate.}
            \item \textbf{DP-based cache size allocation}. We allocate varying cache sizes to different layers by considering diverse factors such as cache hit probabilities, prefetching accuracy, and average expert activation quantities across layers. This allocation aims to minimize the anticipated overhead from on-demand expert loading. We conceptualize this issue as a knapsack problem and employ dynamic programming techniques for its resolution.
        \end{itemize}
    \item Experimental results
        \begin{itemize}
            \item Inference latency with different cache size on different device
            \item Accuracy with different threshold
            \item Ablation Study
                \begin{itemize}
                    \item Predict Accuracy
                    \item On-demand load freq with other method
                    \item cache size visualization
                \end{itemize}
        \end{itemize}
\end{itemize}
